Flexible Mixture Priors for Large Time-varying Parameter Models

Time-varying parameter (TVP) models often assume that the TVPs evolve according to a random walk. This assumption, however, might be questionable since it implies that coefficients change smoothly and in an unbounded manner. In this paper, we relax this assumption by proposing a flexible law of motion for the TVPs in large-scale vector autoregressions (VARs). Instead of imposing a restrictive random walk evolution of the latent states, we carefully design hierarchical mixture priors on the coefficients in the state equation. These priors effectively allow for discriminating between periods where coefficients evolve according to a random walk and times where the TVPs are better characterized by a stationary stochastic process. Moreover, this approach is capable of introducing dynamic sparsity by pushing small parameter changes towards zero if necessary. The merits of the model are illustrated by means of two applications. Using synthetic data we show that our approach yields precise parameter estimates. When applied to US data, the model reveals interesting patterns of low-frequency dynamics in coefficients and forecasts well relative to a wide range of competing models.

==> best_crps_overview.tex <==
\begin{table}[!htb]
{\tiny
\begin{center}
\scalebox{0.9}{
\begin{tabular}{lllllllllllll}
\toprule
\multicolumn{1}{l}{\bfseries Variable}&\multicolumn{1}{c}{}& \multicolumn{3}{c}{\bfseries 1-quarter-ahead}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{\bfseries 1-year-ahead}&\multicolumn{1}{c}{}&\multicolumn{3}{c}{\bfseries 2-years-ahead} \tabularnewline
\cline{3-5} \cline{7-9} \cline{11-13}
\multicolumn{1}{l}{}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Class}&\multicolumn{1}{c}{Subclass}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Class}&\multicolumn{1}{c}{Subclass}&\multicolumn{1}{l}{}&\multicolumn{1}{c}{Size}&\multicolumn{1}{c}{Class}&\multicolumn{1}{c}{Subclass} \tabularnewline
\midrule
\textbf{Density forecasts}& & & & & & & & & & & & \\
& & & & & & & & & & & & \\
\textbf{CRPS ratios} & & & & & & & & & & & & \\[5 pt]
TOT && \texttt{L-VAR}& \texttt{TVP-POOL} & \texttt{FLEX MS-POOL} && \texttt{L-VAR}& \texttt{TVP-POOL} & \texttt{SINGLE} && \texttt{FA-VAR}& \texttt{TVP-POOL} & \texttt{SSVS MIX-SPEC} \\[5 pt]
GDPC1 && \texttt{L-VAR}& \texttt{TVP-POOL} & \texttt{FLEX MIX-SPEC} && \texttt{FA-VAR}& \texttt{TVP-POOL} & \texttt{FLEX MS-POOL} && \texttt{S-VAR}& \texttt{TVP-RW} & \texttt{SINGLE}  \\
\shadeRow CPIAUCSL && \texttt{S-VAR}& \texttt{TVP-MIX} & \texttt{FLEX MIX-SPEC} && \texttt{L-VAR}& \texttt{const. (NG)} &  && \texttt{L-VAR}& \texttt{const. (NG)}   &  \\
UNRATE && \texttt{L-VAR}& \texttt{TVP-POOL} & \texttt{FLEX SSVS MIX-SPEC} && \texttt{L-VAR}& \texttt{TVP-POOL} & \texttt{MS FLEX-POOL} && \texttt{FA-VAR}& \texttt{TVP-POOL}  & \texttt{SINGLE} \\
\shadeRow FEDFUNDS && \texttt{L-VAR}& \texttt{TVP-POOL} & \texttt{FLEX MIX-SPEC} && \texttt{FA-VAR}& \texttt{TVP-RW} & \texttt{FLEX MIX-SPEC} && \texttt{FA-VAR}& \texttt{TVP-POOL}  & \texttt{SSVS MIX-SPEC} \\
\end{tabular}}
\caption{Overview of the best performing models, indicated by bold numbers in \autoref{tab:CRPS}. \label{tab:bestCRPS}}
\end{center}}
\end{table}

==> lps_approx.tex <==
%latex.default(final.tab.2, file = paste0(data.set, "/", substr(type,     6, 20), "_", lps_type, ".tex"), title = "", ctable = FALSE,     rgroupTexCmd = "scshape", rownamesTexCmd = my.rownamesTexCmd,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     rgroup = rgroup, n.rgroup.12 = n.rgroup, caption = "", label = "tab:Dens",     size = "tiny", booktabs = TRUE, rowname = "", numeric.dollar = FALSE,     caption.loc = "bottom", landscape = TRUE)%
\begin{landscape}\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.8}{
\begin{tabular}{lllclllllclllllclllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{2}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries 1-quarter-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries 1-year-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries 2-years-ahead}\tabularnewline
\cline{2-3} \cline{5-9} \cline{11-15} \cline{17-21}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Class}&\multicolumn{1}{c}{Subclass}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{TOT}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{UNRATE}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{TOT}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{UNRATE}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{TOT}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{UNRATE}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   \textbf{FA-VAR}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   const. (Min.)&   &   &    15.07&    13.50**&     5.37&   11.45&    -4.95&   &     34.06*&      7.24**&     2.67&    22.63&    11.27&   &     46.72**&      2.15&      7.20**&     18.94&   \textbf{29.15***}\tabularnewline
   ~~&   const. (NG)&   &   &    26.42*&    15.32***&     8.49&   11.20&     0.51&   &     45.10**&      8.31***&     4.23**&    24.03&    13.46&   &     42.21***&      2.04&      7.21*&     16.56*&    26.22***\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-MIX&   FLEX MIX-SPEC&   &    19.70&    14.66**&    -5.53&   13.30&     8.68***&   &     65.58&      6.46&    -4.88&    43.43&    16.05&   &     66.96&     -1.99&      2.47&     39.12&    12.49\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    34.00&    13.18**&    10.41&   15.95&     6.98*&   &     66.96&      6.06&     1.64&    46.47&    17.98&   &     53.31&     -2.41&     -0.21&     43.63&    15.34\tabularnewline
   ~~&   &   SINGLE&   &    27.29&    11.47**&     0.15&   11.68&    14.36***&   &     65.38*&      4.18&    -5.31&    42.80&    24.12&   &     69.27&     -2.72&      2.24&     40.00&    19.53\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    26.39&    12.95**&    -0.01&   13.66&     6.90***&   &     56.91&      8.34*&    -3.21&    41.85&    10.00&   &     67.66&     -0.53&      3.29&     35.01&     8.41\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-POOL&   FLEX MIX-SPEC&   &    24.66&    14.42***&     6.42&   11.81&     3.93***&   &     47.51**&      9.72**&     3.75*&    24.12&    15.76&   &     71.60*&      3.37&      5.93&     42.66&    27.91**\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    32.91&    15.74***&     7.48*&   12.41&     6.84***&   &     52.94**&     10.11***&     2.26&    28.83&    18.14&   &     62.83**&      3.80&      6.03&     31.27&    28.33**\tabularnewline
   ~~&   &   SINGLE&   &    25.23&    14.56***&     4.71*&   11.31&     5.17***&   &     49.88**&     10.81***&   \textbf{5.09***}&    26.80&    17.41&   &     68.84*&   \textbf{5.00}&   \textbf{7.62}&     41.34&    25.53\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    28.22&    15.20***&     8.07*&   12.24&     3.88***&   &     47.14**&   \textbf{11.26***}&     2.38&    22.50&    17.33&   &     69.25*&      4.85*&      6.25*&     38.28&    27.26*\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-RW&   FLEX MIX-SPEC&   &    45.43&    12.11**&   \textbf{14.70}&   13.87&    16.57***&   &     79.27*&      6.78&    -2.15&    48.33&   \textbf{29.16}&   &   \textbf{87.56}&     -3.84&     -0.03&     57.03&    27.57\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    28.40&    10.98*&    10.97&    8.82&     8.62&   &     59.50&     -0.41&    -6.09&    44.46&    18.29&   &    -43.87&    -70.98**&    -61.96***&     39.26&     1.22\tabularnewline
   ~~&   &   SINGLE&   &    30.08&    14.10**&    -3.35&   14.63&    11.83***&   &     63.59*&      2.84&    -5.19&    35.21&    16.26&   &     44.72&     -7.50&     -0.45&     28.24&    17.17\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    39.98&    12.10**&    12.75&   11.98&    14.58***&   &     76.01*&      4.07&    -2.25&    44.29&    28.09&   &     68.59&     -4.39&      0.85&     37.80&    25.26\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   \textbf{M-VAR}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   const. (Min.)&   &   &    22.01&    13.85&     4.32&   13.27&    -3.89***&   &     88.23&      3.91&     1.52&    56.09&    15.27**&   &     67.33***&     -4.04&      3.70&     27.77&    15.24\tabularnewline
   ~~&   const. (NG)&   &   &    21.56&    17.72***&    -4.95&   15.80&     2.18&   &     95.02*&      6.68***&     4.30&    59.59&    18.95&   &     74.72***&     -1.69&      6.67&     26.15*&    18.51**\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-MIX&   FLEX MIX-SPEC&   &    26.89&    13.81*&     1.42&   17.03&     4.41&   &     69.88&      6.73&    -7.11&    57.05&     5.05&   &     30.88&    -12.94*&    -15.52**&     39.47&    -3.64\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    25.54&    11.19&     4.76&   14.34&     6.91&   &     73.00&      4.16&     0.19&    56.00&     6.80&   &     47.29&    -16.92&     -6.57&     52.38&    -0.85\tabularnewline
   ~~&   &   SINGLE&   &    32.27&    13.25*&     3.27&   15.07&    10.83&   &     78.51&      7.46&    -0.42&    55.90&     7.97&   &     60.22&    -10.79&     -2.73&     47.53&     5.22\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    14.60&    13.07*&   -12.32&   14.22&    10.17&   &     73.35&      6.33&    -7.24&    54.58&     7.92&   &     61.54&     -8.23&     -2.70&     51.53&     1.06\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-POOL&   FLEX MIX-SPEC&   &    43.60&    17.51***&    -1.62&   17.34&    19.88***&   &     95.97*&      5.82**&     0.58&    58.85&    25.61&   &     84.77**&     -2.29&      1.04&     47.91&    18.23*\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    41.28&   \textbf{18.20***}&    -7.43&   18.54&    19.76***&   &     96.39*&      7.17**&     1.13&    60.77&    23.95&   &     77.50**&     -3.39&      0.80&     44.28&    18.60\tabularnewline
   ~~&   &   SINGLE&   &   \textbf{46.90}&    17.22***&    -1.73&   \textbf{18.92}&   \textbf{20.85***}&   &   \textbf{99.38*}&      8.52***&     3.63&    59.84&    25.13&   &     87.13**&     -0.39&      2.81&     49.31&    16.30\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    39.69&    17.19**&    -6.53&   17.61&    20.84***&   &     98.54*&      5.88**&     0.01&   \textbf{63.02}&    26.54&   &     81.21**&     -3.82&      1.23&     45.53&    18.98*\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-RW&   FLEX MIX-SPEC&   &     9.17&    11.37*&   -16.52&   10.88&    11.67&   &     79.91&      4.12&     0.39&    49.28&    18.53&   &     63.71&    -16.50&     -8.81&   \textbf{57.58}&    13.71\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   -33.72&     5.93&   -11.17&    2.93**&   -22.00***&   &    -40.25&    -26.32&   -31.31***&    33.80&   -18.28&   &   -336.23**&   -164.50***&   -165.83***&     -0.12&   -90.63**\tabularnewline
   ~~&   &   SINGLE&   &    29.41&    12.42&     7.88&   12.72&     7.38&   &     57.15&      4.41&    -2.20&    50.99&    -6.65&   &      4.57&    -20.29***&    -19.92**&     35.39&   -13.36**\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    -2.34&    11.02&   -24.01&   11.94&    12.13**&   &     78.13&      3.97&     1.50&    47.92&    14.64&   &     61.15&    -12.15&     -2.59&     46.42&     7.50\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   \textbf{S-VAR}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
\shadeBench   ~~&   const. (Min.)&   &   &   -40.99&   -84.68&   -94.83&   43.06&    82.89&   &   -301.86&   -101.39&   -89.58&   -94.88&   -34.89&   &   -430.04&    -94.77&    -93.19&   -166.90&   -85.97\tabularnewline
   ~~&   const. (NG)&   &   &    -5.43&     0.08&    -3.40&   -0.04**&     0.41**&   &      1.66&     -1.73&     2.87&    -2.87&     2.01&   &     -9.36&     -2.17&      1.53&     -5.58&    -1.72\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-MIX&   FLEX MIX-SPEC&   &    12.37&     4.16*&    -1.56&    5.62&     9.18***&   &     22.96&      1.54&    -7.94&    15.42&     3.45&   &     21.96&     -1.40&      4.12&      6.59&    -6.28\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    12.80&     3.47&     4.06&    7.92&     3.07**&   &     12.36&     -1.02&   -14.53&    21.11&     0.05*&   &     32.38&     -4.76&      4.63&     23.37&    -5.85\tabularnewline
   ~~&   &   SINGLE&   &   -23.27&     1.68&   -29.22&    1.59&    10.09***&   &     21.94&      3.94&    -7.46&     9.32&     4.16*&   &     20.01&     -5.34&      0.17&      5.87&     0.28\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    11.02&     3.79*&     9.32*&    3.34&     3.32***&   &     28.41&      1.64&    -6.54&    16.13&     3.76&   &     49.75&     -1.31&      5.37&     21.81&    -0.60\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-POOL&   FLEX MIX-SPEC&   &    -3.87&     2.22**&     1.85&    0.20&    -6.17&   &     23.86**&      3.39**&     0.33&     7.72*&     9.52&   &      8.88&     -1.66&      2.09&      9.48&    -0.78\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    -3.70&     2.46*&    -1.87&    1.34&    -4.80*&   &     13.90&      2.08&     1.44&     4.43**&     9.05&   &     20.15&     -1.39&      3.66&     13.03&     1.72\tabularnewline
   ~~&   &   SINGLE&   &    -5.13&     1.70**&    -2.30&    1.13&    -1.68**&   &     13.57&      0.43&     1.21&     9.22&     9.03&   &     11.61&     -3.11&      2.75&     15.94&    -3.52\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &     9.76&     2.15**&     6.20**&    1.63&     0.03**&   &     12.06&      0.25&     1.47&     8.97**&     7.10&   &      8.04&     -3.38&      3.21&     16.26&    -2.33\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-RW&   FLEX MIX-SPEC&   &    16.56&     2.05&     8.65**&    3.36*&     6.12***&   &     38.60*&      1.12&    -0.49&    19.98&     9.89&   &     49.06&     -6.14*&      1.75&     26.27&     7.35\tabularnewline
   ~~&   &   FLEX MS-POOL&   &    13.88&     2.35&    10.07&    2.43*&     8.74*&   &     25.84&      0.51&   -11.30&    22.21&     7.85&   &    -25.24&    -33.51***&    -33.59&      7.78&   -10.36\tabularnewline
   ~~&   &   SINGLE&   &   -10.32**&     5.96**&   -12.08&    3.81&     4.70***&   &     15.08&      1.68&   -11.08&     9.43&    11.50&   &     -2.37&      0.68&     -2.13&     -0.18&     4.66\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &    12.40&     1.34&     5.50*&    1.07&    10.21***&   &     23.97*&     -0.30&    -2.17&     9.25&     8.65&   &     20.52&     -6.66&      2.13&      2.75&     1.77\tabularnewline
\bottomrule
\end{tabular}}
\caption{\label{tab:LPS}}\end{center}}
\end{table}\end{landscape}


==> rmse_lps_approx.tex <==
%latex.default(final.tab.full, file = paste0(data.set, "/", type,     "_", lps_type, ".tex"), title = "", ctable = FALSE, rgroupTexCmd = "scshape",     rownamesTexCmd = my.rownamesTexCmd, n.cgroup = n.cgroup,     cgroup = cgroup, colheads = colheads, rgroup = rgroup, n.rgroup.full = n.rgroup,     caption = "", label = "tab:PointDens", size = "tiny", booktabs = TRUE,     rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{lllclllllclllllclllll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{2}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries 1-quarter-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries 1-year-ahead}&\multicolumn{1}{c}{\bfseries }&\multicolumn{5}{c}{\bfseries 2-years-ahead}\tabularnewline
\cline{2-3} \cline{5-9} \cline{11-15} \cline{17-21}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Class}&\multicolumn{1}{c}{Subclass}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{TOT}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{UNRATE}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{TOT}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{UNRATE}&\multicolumn{1}{c}{FEDFUNDS}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{TOT}&\multicolumn{1}{c}{GDPC1}&\multicolumn{1}{c}{CPIAUCSL}&\multicolumn{1}{c}{UNRATE}&\multicolumn{1}{c}{FEDFUNDS}\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   \textbf{FA-VAR}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   const. (Min.)&   &   &   0.91*&   0.87&   0.94&   0.79&   1.22&   &   0.92**&   0.84*&   1.03&   0.80&   1.11&   &   0.93*&   1.00&   1.04&   0.86&   0.78***\tabularnewline
   ~~&   &   &   &   (15.07)&   (13.50**)&   (5.37)&   (11.45)&   (-4.95)&   &   (34.06*)&   (7.24**)&   (2.67)&   (22.63)&   (11.27)&   &   (46.72**)&   (2.15)&   (7.20**)&   (18.94)&   (\textbf{29.15***})\tabularnewline
   ~~&   const. (NG)&   &   &   0.88**&   0.81*&   0.95&   0.80&   1.14&   &   0.90**&   0.84**&   0.99&   0.81&   1.02&   &   0.92&   1.00&   1.01&   0.87&   0.75**\tabularnewline
   ~~&   &   &   &   (26.42*)&   (15.32***)&   (8.49)&   (11.20)&   (0.51)&   &   (45.10**)&   (8.31***)&   (4.23**)&   (24.03)&   (13.46)&   &   (42.21***)&   (2.04)&   (7.21*)&   (16.56*)&   (26.22***)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-MIX&   FLEX MIX-SPEC&   &   0.89**&   0.80*&   0.96&   0.81&   0.91&   &   0.95*&   0.93&   0.99&   0.89&   0.98&   &   1.00&   \textbf{0.86}&   1.09&   1.06&   0.93\tabularnewline
   ~~&   &   &   &   (19.70)&   (14.66**)&   (-5.53)&   (13.30)&   (8.68***)&   &   (65.58)&   (6.46)&   (-4.88)&   (43.43)&   (16.05)&   &   (66.96)&   (-1.99)&   (2.47)&   (39.12)&   (12.49)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.91**&   0.83&   0.99&   0.78&   0.88&   &   0.91&   0.90&   0.99&   0.80&   0.83*&   &   0.94&   0.97&   1.01&   0.91&   0.89\tabularnewline
   ~~&   &   &   &   (34.00)&   (13.18**)&   (10.41)&   (15.95)&   (6.98*)&   &   (66.96)&   (6.06)&   (1.64)&   (46.47)&   (17.98)&   &   (53.31)&   (-2.41)&   (-0.21)&   (43.63)&   (15.34)\tabularnewline
   ~~&   &   SINGLE&   &   0.92*&   0.83&   1.01&   0.79&   0.85**&   &   0.92*&   0.87&   1.02&   0.82&   0.87&   &   0.96&   0.93&   1.11&   0.93&   0.87\tabularnewline
   ~~&   &   &   &   (27.29)&   (11.47**)&   (0.15)&   (11.68)&   (14.36***)&   &   (65.38*)&   (4.18)&   (-5.31)&   (42.80)&   (24.12)&   &   (69.27)&   (-2.72)&   (2.24)&   (40.00)&   (19.53)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.90**&   0.83&   0.96&   0.79&   0.95&   &   0.91*&   0.88&   0.99&   0.83&   0.96&   &   0.96&   0.96&   1.09&   0.88&   0.92\tabularnewline
   ~~&   &   &   &   (26.39)&   (12.95**)&   (-0.01)&   (13.66)&   (6.90***)&   &   (56.91)&   (8.34*)&   (-3.21)&   (41.85)&   (10.00)&   &   (67.66)&   (-0.53)&   (3.29)&   (35.01)&   (8.41)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-POOL&   FLEX MIX-SPEC&   &   0.88**&   0.79*&   0.95&   0.77&   1.06&   &   0.87**&   \textbf{0.80**}&   0.99&   0.77&   0.97&   &   0.89&   0.97&   1.02&   0.81&   0.73*\tabularnewline
   ~~&   &   &   &   (24.66)&   (14.42***)&   (6.42)&   (11.81)&   (3.93***)&   &   (47.51**)&   (9.72**)&   (3.75*)&   (24.12)&   (15.76)&   &   (71.60*)&   (3.37)&   (5.93)&   (42.66)&   (27.91**)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.88**&   0.78*&   0.96&   0.76&   1.07&   &   0.87**&   0.80**&   0.97&   0.77&   0.97&   &   0.88&   0.96&   0.99&   0.82&   0.74*\tabularnewline
   ~~&   &   &   &   (32.91)&   (15.74***)&   (7.48*)&   (12.41)&   (6.84***)&   &   (52.94**)&   (10.11***)&   (2.26)&   (28.83)&   (18.14)&   &   (62.83**)&   (3.80)&   (6.03)&   (31.27)&   (28.33**)\tabularnewline
   ~~&   &   SINGLE&   &   0.87**&   0.79*&   0.95&   0.78&   1.06&   &   0.87**&   0.81**&   0.98&   0.78&   0.98&   &   0.88&   0.95*&   1.01&   0.81&   0.74*\tabularnewline
   ~~&   &   &   &   (25.23)&   (14.56***)&   (4.71*)&   (11.31)&   (5.17***)&   &   (49.88**)&   (10.81***)&   (\textbf{5.09***})&   (26.80)&   (17.41)&   &   (68.84*)&   (\textbf{5.00})&   (\textbf{7.62})&   (41.34)&   (25.53)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.88***&   0.80*&   0.94&   0.76&   1.05&   &   0.88**&   0.80**&   0.99&   0.78&   0.98&   &   \textbf{0.88}&   0.95*&   1.01&   \textbf{0.81}&   \textbf{0.73*}\tabularnewline
   ~~&   &   &   &   (28.22)&   (15.20***)&   (8.07*)&   (12.24)&   (3.88***)&   &   (47.14**)&   (\textbf{11.26***})&   (2.38)&   (22.50)&   (17.33)&   &   (69.25*)&   (4.85*)&   (6.25*)&   (38.28)&   (27.26*)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-RW&   FLEX MIX-SPEC&   &   0.89**&   0.82&   0.95&   0.77&   0.89**&   &   0.88*&   0.86&   0.98&   0.76&   0.81**&   &   0.93&   1.00&   0.99&   0.88&   0.79\tabularnewline
   ~~&   &   &   &   (45.43)&   (12.11**)&   (\textbf{14.70})&   (13.87)&   (16.57***)&   &   (79.27*)&   (6.78)&   (-2.15)&   (48.33)&   (\textbf{29.16})&   &   (\textbf{87.56})&   (-3.84)&   (-0.03)&   (57.03)&   (27.57)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.91*&   0.85&   0.98&   0.81&   0.95&   &   0.92&   0.90&   1.01&   0.80&   0.84*&   &   0.96&   1.00&   1.01&   0.94&   0.88\tabularnewline
   ~~&   &   &   &   (28.40)&   (10.98*)&   (10.97)&   (8.82)&   (8.62)&   &   (59.50)&   (-0.41)&   (-6.09)&   (44.46)&   (18.29)&   &   (-43.87)&   (-70.98**)&   (-61.96***)&   (39.26)&   (1.22)\tabularnewline
   ~~&   &   SINGLE&   &   0.90**&   0.82&   0.98&   0.81&   0.95&   &   1.03&   1.01&   1.03&   1.00&   1.23&   &   1.20&   0.89&   1.25&   1.31*&   1.30\tabularnewline
   ~~&   &   &   &   (30.08)&   (14.10**)&   (-3.35)&   (14.63)&   (11.83***)&   &   (63.59*)&   (2.84)&   (-5.19)&   (35.21)&   (16.26)&   &   (44.72)&   (-7.50)&   (-0.45)&   (28.24)&   (17.17)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.91*&   0.85&   0.98&   0.80&   \textbf{0.83**}&   &   0.91&   0.90&   0.98&   0.82&   \textbf{0.79**}&   &   0.95&   0.99&   1.01&   0.94&   0.82\tabularnewline
   ~~&   &   &   &   (39.98)&   (12.10**)&   (12.75)&   (11.98)&   (14.58***)&   &   (76.01*)&   (4.07)&   (-2.25)&   (44.29)&   (28.09)&   &   (68.59)&   (-4.39)&   (0.85)&   (37.80)&   (25.26)\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   \textbf{M-VAR}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   const. (Min.)&   &   &   1.02&   0.99&   1.05&   0.72&   1.52&   &   0.92**&   0.93&   0.95*&   0.79&   1.00&   &   0.97**&   1.02&   0.98&   0.95&   0.88**\tabularnewline
   ~~&   &   &   &   (22.01)&   (13.85)&   (4.32)&   (13.27)&   (-3.89***)&   &   (88.23)&   (3.91)&   (1.52)&   (56.09)&   (15.27**)&   &   (67.33***)&   (-4.04)&   (3.70)&   (27.77)&   (15.24)\tabularnewline
   ~~&   const. (NG)&   &   &   0.91**&   0.85&   0.96&   0.71&   1.10&   &   0.88***&   0.89*&   0.92**&   0.74&   0.98&   &   0.92**&   1.00&   0.97&   0.89&   0.79**\tabularnewline
   ~~&   &   &   &   (21.56)&   (17.72***)&   (-4.95)&   (15.80)&   (2.18)&   &   (95.02*)&   (6.68***)&   (4.30)&   (59.59)&   (18.95)&   &   (74.72***)&   (-1.69)&   (6.67)&   (26.15*)&   (18.51**)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-MIX&   FLEX MIX-SPEC&   &   1.02&   0.90&   1.10&   0.71&   2.20&   &   0.87**&   0.80*&   0.94&   0.79&   1.05&   &   0.93&   0.96&   0.98&   0.89&   0.89\tabularnewline
   ~~&   &   &   &   (26.89)&   (13.81*)&   (1.42)&   (17.03)&   (4.41)&   &   (69.88)&   (6.73)&   (-7.11)&   (57.05)&   (5.05)&   &   (30.88)&   (-12.94*)&   (-15.52**)&   (39.47)&   (-3.64)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   1.06&   0.92&   1.19&   0.71&   1.51&   &   0.89**&   0.87&   0.93&   0.79&   1.06&   &   1.13&   1.53&   0.95&   0.92&   1.01\tabularnewline
   ~~&   &   &   &   (25.54)&   (11.19)&   (4.76)&   (14.34)&   (6.91)&   &   (73.00)&   (4.16)&   (0.19)&   (56.00)&   (6.80)&   &   (47.29)&   (-16.92)&   (-6.57)&   (52.38)&   (-0.85)\tabularnewline
   ~~&   &   SINGLE&   &   0.91*&   0.84&   0.97&   0.74&   0.91**&   &   0.87**&   0.83*&   0.94&   0.83&   0.88*&   &   0.94&   0.97&   0.99&   0.92&   0.86\tabularnewline
   ~~&   &   &   &   (32.27)&   (13.25*)&   (3.27)&   (15.07)&   (10.83)&   &   (78.51)&   (7.46)&   (-0.42)&   (55.90)&   (7.97)&   &   (60.22)&   (-10.79)&   (-2.73)&   (47.53)&   (5.22)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.96&   0.98&   0.93&   0.72&   1.19&   &   0.89&   0.85&   0.97&   0.79&   1.00&   &   0.95&   0.95&   1.06&   0.89&   0.90\tabularnewline
   ~~&   &   &   &   (14.60)&   (13.07*)&   (-12.32)&   (14.22)&   (10.17)&   &   (73.35)&   (6.33)&   (-7.24)&   (54.58)&   (7.92)&   &   (61.54)&   (-8.23)&   (-2.70)&   (51.53)&   (1.06)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-POOL&   FLEX MIX-SPEC&   &   \textbf{0.87***}&   \textbf{0.78**}&   0.95&   0.69&   0.87***&   &   0.87**&   0.87&   0.93&   0.74&   0.89**&   &   0.90&   0.97&   1.00&   0.83&   0.81**\tabularnewline
   ~~&   &   &   &   (43.60)&   (17.51***)&   (-1.62)&   (17.34)&   (19.88***)&   &   (95.97*)&   (5.82**)&   (0.58)&   (58.85)&   (25.61)&   &   (84.77**)&   (-2.29)&   (1.04)&   (47.91)&   (18.23*)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.88***&   0.81**&   0.94&   \textbf{0.66*}&   0.87***&   &   0.86**&   0.85*&   0.94&   \textbf{0.71}&   0.90**&   &   0.90&   0.97&   1.00&   0.83&   0.79**\tabularnewline
   ~~&   &   &   &   (41.28)&   (\textbf{18.20***})&   (-7.43)&   (18.54)&   (19.76***)&   &   (96.39*)&   (7.17**)&   (1.13)&   (60.77)&   (23.95)&   &   (77.50**)&   (-3.39)&   (0.80)&   (44.28)&   (18.60)\tabularnewline
   ~~&   &   SINGLE&   &   0.88***&   0.80**&   0.95&   0.67*&   1.64&   &   \textbf{0.85**}&   0.85*&   \textbf{0.90*}&   0.73&   0.91**&   &   0.89*&   0.95&   0.98&   0.83&   0.79**\tabularnewline
   ~~&   &   &   &   (\textbf{46.90})&   (17.22***)&   (-1.73)&   (\textbf{18.92})&   (\textbf{20.85***})&   &   (\textbf{99.38*})&   (8.52***)&   (3.63)&   (59.84)&   (25.13)&   &   (87.13**)&   (-0.39)&   (2.81)&   (49.31)&   (16.30)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.88**&   0.82**&   0.95&   0.68&   0.87***&   &   0.87**&   0.86&   0.95&   0.72&   0.90**&   &   0.90&   0.96&   1.00&   0.83&   0.79**\tabularnewline
   ~~&   &   &   &   (39.69)&   (17.19**)&   (-6.53)&   (17.61)&   (20.84***)&   &   (98.54*)&   (5.88**)&   (0.01)&   (\textbf{63.02})&   (26.54)&   &   (81.21**)&   (-3.82)&   (1.23)&   (45.53)&   (18.98*)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-RW&   FLEX MIX-SPEC&   &   0.97&   0.98&   0.97&   0.73&   1.07&   &   0.87**&   0.84&   0.95&   0.79&   0.92*&   &   0.95&   0.97&   0.99&   0.93&   0.87\tabularnewline
   ~~&   &   &   &   (9.17)&   (11.37*)&   (-16.52)&   (10.88)&   (11.67)&   &   (79.91)&   (4.12)&   (0.39)&   (49.28)&   (18.53)&   &   (63.71)&   (-16.50)&   (-8.81)&   (\textbf{57.58})&   (13.71)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.99&   0.96&   1.02&   0.75&   1.28&   &   0.90&   0.88&   0.93&   0.83&   1.01&   &   0.98&   1.01&   1.02&   0.95&   0.95\tabularnewline
   ~~&   &   &   &   (-33.72)&   (5.93)&   (-11.17)&   (2.93**)&   (-22.00***)&   &   (-40.25)&   (-26.32)&   (-31.31***)&   (33.80)&   (-18.28)&   &   (-336.23**)&   (-164.50***)&   (-165.83***)&   (-0.12)&   (-90.63**)\tabularnewline
   ~~&   &   SINGLE&   &   1.23&   1.10&   1.35&   0.75&   1.76&   &   0.91*&   0.83&   0.96**&   0.85&   1.22&   &   0.94&   0.90&   0.95&   0.96&   0.94\tabularnewline
   ~~&   &   &   &   (29.41)&   (12.42)&   (7.88)&   (12.72)&   (7.38)&   &   (57.15)&   (4.41)&   (-2.20)&   (50.99)&   (-6.65)&   &   (4.57)&   (-20.29***)&   (-19.92**)&   (35.39)&   (-13.36**)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.94&   0.92&   0.95&   0.73&   1.17&   &   0.89*&   0.86&   0.95&   0.83&   0.95&   &   0.96&   0.96&   0.96&   0.96&   0.95\tabularnewline
   ~~&   &   &   &   (-2.34)&   (11.02)&   (-24.01)&   (11.94)&   (12.13**)&   &   (78.13)&   (3.97)&   (1.50)&   (47.92)&   (14.64)&   &   (61.15)&   (-12.15)&   (-2.59)&   (46.42)&   (7.50)\tabularnewline
\midrule
{\scshape }&&&&&&&&&&&&&&&&&&&&\tabularnewline
   ~~&   \textbf{S-VAR}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
\shadeBench   ~~&   const. (Min.)&   &   &   0.60&   0.83&   0.85&   0.15&   0.11&   &   0.76&   1.00&   0.87&   0.62&   0.41&   &   0.91&   0.93&   0.85&   1.10&   0.73\tabularnewline
\shadeBench   ~~&   &   &   &   (-40.99)&   (-84.68)&   (-94.83)&   (43.06)&   (82.89)&   &   (-301.86)&   (-101.39)&   (-89.58)&   (-94.88)&   (-34.89)&   &   (-430.04)&   (-94.77)&   (-93.19)&   (-166.90)&   (-85.97)\tabularnewline
   ~~&   const. (NG)&   &   &   0.99**&   0.99*&   0.99&   1.00&   1.01&   &   0.96**&   0.94*&   0.98&   0.98*&   0.98&   &   0.97&   0.99&   0.98&   0.97**&   0.95\tabularnewline
   ~~&   &   &   &   (-5.43)&   (0.08)&   (-3.40)&   (-0.04**)&   (0.41**)&   &   (1.66)&   (-1.73)&   (2.87)&   (-2.87)&   (2.01)&   &   (-9.36)&   (-2.17)&   (1.53)&   (-5.58)&   (-1.72)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-MIX&   FLEX MIX-SPEC&   &   0.93**&   0.94*&   \textbf{0.92}&   0.92&   0.93**&   &   0.89&   0.82&   0.94&   0.92&   0.93&   &   0.93&   0.89&   1.00&   0.92&   0.92\tabularnewline
   ~~&   &   &   &   (12.37)&   (4.16*)&   (-1.56)&   (5.62)&   (9.18***)&   &   (22.96)&   (1.54)&   (-7.94)&   (15.42)&   (3.45)&   &   (21.96)&   (-1.40)&   (4.12)&   (6.59)&   (-6.28)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.96&   0.97&   0.95&   0.92&   0.87&   &   0.94&   0.94&   0.96&   0.91&   0.97&   &   0.96&   0.97&   1.01&   0.92&   0.95\tabularnewline
   ~~&   &   &   &   (12.80)&   (3.47)&   (4.06)&   (7.92)&   (3.07**)&   &   (12.36)&   (-1.02)&   (-14.53)&   (21.11)&   (0.05*)&   &   (32.38)&   (-4.76)&   (4.63)&   (23.37)&   (-5.85)\tabularnewline
   ~~&   &   SINGLE&   &   0.97&   0.98&   0.97&   0.96&   0.85*&   &   0.93&   0.91&   0.95&   0.95&   0.96&   &   0.96&   0.96&   0.99&   0.94&   0.93\tabularnewline
   ~~&   &   &   &   (-23.27)&   (1.68)&   (-29.22)&   (1.59)&   (10.09***)&   &   (21.94)&   (3.94)&   (-7.46)&   (9.32)&   (4.16*)&   &   (20.01)&   (-5.34)&   (0.17)&   (5.87)&   (0.28)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.95**&   0.97&   0.94**&   0.97&   0.95***&   &   0.91&   0.87&   0.95&   0.94&   0.92&   &   0.95&   0.93&   1.01&   0.94&   0.93\tabularnewline
   ~~&   &   &   &   (11.02)&   (3.79*)&   (9.32*)&   (3.34)&   (3.32***)&   &   (28.41)&   (1.64)&   (-6.54)&   (16.13)&   (3.76)&   &   (49.75)&   (-1.31)&   (5.37)&   (21.81)&   (-0.60)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-POOL&   FLEX MIX-SPEC&   &   0.98***&   0.97**&   0.98&   0.96&   0.98&   &   0.96**&   0.94&   0.98&   0.94&   0.94&   &   0.95&   0.99&   0.98&   0.93&   0.91\tabularnewline
   ~~&   &   &   &   (-3.87)&   (2.22**)&   (1.85)&   (0.20)&   (-6.17)&   &   (23.86**)&   (3.39**)&   (0.33)&   (7.72*)&   (9.52)&   &   (8.88)&   (-1.66)&   (2.09)&   (9.48)&   (-0.78)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.98**&   0.96**&   0.99&   0.94*&   0.99&   &   0.96**&   0.95*&   0.99&   0.94&   0.95&   &   0.96&   1.00&   0.97&   0.93&   0.91\tabularnewline
   ~~&   &   &   &   (-3.70)&   (2.46*)&   (-1.87)&   (1.34)&   (-4.80*)&   &   (13.90)&   (2.08)&   (1.44)&   (4.43**)&   (9.05)&   &   (20.15)&   (-1.39)&   (3.66)&   (13.03)&   (1.72)\tabularnewline
   ~~&   &   SINGLE&   &   0.98**&   0.98&   0.98&   0.95&   0.98&   &   0.96**&   0.94*&   0.98**&   0.94&   0.95&   &   0.95&   1.00&   0.98&   0.92&   0.91\tabularnewline
   ~~&   &   &   &   (-5.13)&   (1.70**)&   (-2.30)&   (1.13)&   (-1.68**)&   &   (13.57)&   (0.43)&   (1.21)&   (9.22)&   (9.03)&   &   (11.61)&   (-3.11)&   (2.75)&   (15.94)&   (-3.52)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.97***&   0.97**&   0.98&   0.95&   0.97*&   &   0.95**&   0.94&   0.97&   0.93&   0.95&   &   0.95&   1.00&   0.98&   0.92&   0.91\tabularnewline
   ~~&   &   &   &   (9.76)&   (2.15**)&   (6.20**)&   (1.63)&   (0.03**)&   &   (12.06)&   (0.25)&   (1.47)&   (8.97**)&   (7.10)&   &   (8.04)&   (-3.38)&   (3.21)&   (16.26)&   (-2.33)\tabularnewline
   ~~&   \textbf{}&   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   &   \tabularnewline
   ~~&   TVP-RW&   FLEX MIX-SPEC&   &   0.96**&   0.97&   0.95&   0.96&   0.93**&   &   0.93**&   0.93*&   0.91&   0.96&   0.95&   &   0.95&   0.97&   \textbf{0.94}&   0.95&   0.95\tabularnewline
   ~~&   &   &   &   (16.56)&   (2.05)&   (8.65**)&   (3.36*)&   (6.12***)&   &   (38.60*)&   (1.12)&   (-0.49)&   (19.98)&   (9.89)&   &   (49.06)&   (-6.14*)&   (1.75)&   (26.27)&   (7.35)\tabularnewline
   ~~&   &   FLEX MS-POOL&   &   0.97&   0.97&   0.96&   1.00&   0.85**&   &   0.95&   0.93&   0.97&   0.97&   0.94&   &   0.96&   0.95&   1.01&   0.96&   0.93\tabularnewline
   ~~&   &   &   &   (13.88)&   (2.35)&   (10.07)&   (2.43*)&   (8.74*)&   &   (25.84)&   (0.51)&   (-11.30)&   (22.21)&   (7.85)&   &   (-25.24)&   (-33.51***)&   (-33.59)&   (7.78)&   (-10.36)\tabularnewline
   ~~&   &   SINGLE&   &   0.94*&   0.91*&   0.98&   0.92&   0.85***&   &   0.89&   0.83&   0.96&   0.93&   0.89&   &   0.94&   0.89&   1.01&   0.96&   0.85\tabularnewline
   ~~&   &   &   &   (-10.32**)&   (5.96**)&   (-12.08)&   (3.81)&   (4.70***)&   &   (15.08)&   (1.68)&   (-11.08)&   (9.43)&   (11.50)&   &   (-2.37)&   (0.68)&   (-2.13)&   (-0.18)&   (4.66)\tabularnewline
   ~~&   &   SSVS MIX-SPEC&   &   0.99&   1.00&   0.97&   0.99&   0.89&   &   0.94&   0.94&   0.93&   0.98&   0.96&   &   0.97&   0.96&   0.97&   0.98&   0.96\tabularnewline
   ~~&   &   &   &   (12.40)&   (1.34)&   (5.50*)&   (1.07)&   (10.21***)&   &   (23.97*)&   (-0.30)&   (-2.17)&   (9.25)&   (8.65)&   &   (20.52)&   (-6.66)&   (2.13)&   (2.75)&   (1.77)\tabularnewline
\bottomrule
\end{tabular}}
\caption{\label{tab:PointDens}}\end{center}}
\end{table}

